External-Wrench Estimation for Aerial Robots Exploiting a Learned Model

This paper presents an external wrench estimator that uses a hybrid dynamics model consisting of a first-principles model and a neural network. This framework addresses one of the limitations of the state-of-the-art model-based wrench observers: the wrench estimation of these observers comprises the external wrench (e.g. collision, physical interaction, wind); in addition to residual wrench (e.g. model parameters uncertainty or unmodeled dynamics). This is a problem if these wrench estimations are to be used as wrench feedback to a force controller, for example. In the proposed framework, a neural network is combined with a first-principles model to estimate the residual dynamics arising from unmodeled dynamics and parameters uncertainties, then, the hybrid trained model is used to estimate the external wrench, leading to a wrench estimation that has smaller contributions from the residual dynamics, and affected more by the external wrench. This method is validated with numerical simulations of an aerial robot in different flying scenarios and different types of residual dynamics, and the statistical analysis of the results shows that the wrench estimation error has improved significantly compared to a model-based wrench observer using only a first-principles model.

==> old_things/old_section_III.tex <==
\section{Knowledge-based Neural ODEs for Learning the Residual Dynamics of an Aerial Robot} \label{sec-KNODE}

Neural Ordinary Differential Equations (NODE) was proposed by Chen et al. \cite{chen_neural_2018} to combine differential equations and their numerical solvers with neural networks. Then it was extended by Jihao et al. in \cite{jiahao_knowledge-based_2021} to incorporate FP models to learn the nonlinear and chaotic systems. The authors denoted this approach with Knowledge-based Neural ODEs (KNODE). The authors show how KNODE models can generalize better than other NN architectures; are better in extrapolating beyond the training data; are less prone to over-fitting; and are robust to noisy and irregularly sampled data. For these reasons, KNODE was chosen as the NN architecture for this work.

In this section, the problem of learning the residual dynamics of an MRAV will be explained, inspired by the work in \cite{jiahao_knowledge-based_2021,chee_knode-mpc_2022}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/KNODE-training.pdf}
    \caption{Block diagram of the KNODE Model and its training procedure. This example is for a prediction horizon $\alpha = 1$. The two models calculate the predicted dynamics of the system based on the initial condition of the states $\boldsymbol{x}(t)$ and the input $\boldsymbol{u}(t)$, then the predictions of the two models are combined and integrated using a numerical integrator (such as Runge-Kutta). The model is trained by optimizing the network parameters based on the prediction error between the KNODE next step prediction $\hat{\boldsymbol{x}}(t+1)$ and the real next step states $\boldsymbol{x}(t+1)$.}
    \label{fig-KNODE-learning-simple}
\end{figure}

\subsection{Problem Setup}

\begin{comment}
  
, after we agree on this I will modify it to resolve some issues:
\begin{itemize}
    \item The notation has been slightly changed to better clarify some aspects.
    \item In \cite{jiahao_knowledge-based_2021} the system is suited to learn autonomous system's dynamics, our system is non autonomous therefore I had to change few things in order to fit the method in our framework.
    \item For know I don't consider downsampling because there is no need to that yet. I will make a chapter to discuss this if needed.
    \item I left the description of \( \mathbf{M}_{out} \) just for you to respect the original idea, but as already discussed we don't need it because we assume that the knowledge we have of the real model is reliable and the uncertainty space is separable from the model. In our framework \( \mathbf{M}_{out} \) can be sobstituted by an add node.
    
\end{itemize}  
\end{comment}

% Assume that the real-world system is described by the following function
% \begin{equation*}
%     \dot{\boldsymbol{x}} = f\left(\boldsymbol{x},\boldsymbol{u}\right)
% \end{equation*}
% where \(f : \mathbb{R}^n\times\mathbb{R}^m\rightarrow\mathbb{R}^n\) denotes the real dynamics that is partially known from the physical description of the system.

% The partial knowledge of the dynamics of the real system in this work we will denote with 
% \begin{equation}
%     \label{partial_knowledge}
%     \tilde{f}(\boldsymbol{x},\boldsymbol{u}) = f\left(\boldsymbol{x},\boldsymbol{u}\right) - \boldsymbol{\phi}
% \end{equation}
% where, \(\boldsymbol{\phi}\) represent the unmodeled residual dynamics of the system, that represents epistemic uncertainties.

Defining the states and the input to the MRAV system as $\boldsymbol{x}$ and $\boldsymbol{u}$, such that:
\begin{equation}
    \boldsymbol{x} \coloneq  \begin{bmatrix}
        \twist & \mathbf{R}
    \end{bmatrix}, \quad \boldsymbol{u} \coloneq  \boldsymbol{\gamma}
\end{equation}

% \begin{equation}
%     \boldsymbol{x} \coloneq 
%         \twist
%     , 
%     \quad
%     \boldsymbol{u} \coloneq
%         \boldsymbol{\gamma}
% \end{equation}

While the real systems dynamics is described as in \eqref{eq-real-dynamics-with-tilde-phi}, the dynamics of the learned model that includes both the FP model and the learned residual dynamics can be described using the following notation:
\begin{equation}
    \label{eq-f-hat-KNODE}
    \dot{\hat{\boldsymbol{x}}} = \hat{f}(\hat{\boldsymbol{x}},\boldsymbol{u},\boldsymbol{\phi}_{\theta}(\hat{\boldsymbol{x}},\boldsymbol{u})) = \tilde{f}(\hat{\boldsymbol{x}},\boldsymbol{u}) + \boldsymbol{\phi}_{\theta}(\hat{\boldsymbol{x}},\boldsymbol{u})
\end{equation}
where \(\hat{f}: \mathbb{R}^6\times\mathbb{R}^{3\times3}\times\mathbb{R}^6\rightarrow\mathbb{R}^6\) is the KNODE model and \(\boldsymbol{\phi}_\theta: \mathbb{R}^6\times\mathbb{R}^{3\times3}\times\mathbb{R}^6\rightarrow\mathbb{R}^6\) is a NN that approximates the residual dynamics. The weights of the NN are denoted with \(\boldsymbol{\theta}\).

% In this setup, as depicted in the blue square in Fig. \ref{fig:resnet}, the function \(\hat{f}\) incorporates some known dynamics of the system along with a trained neural network model, these outputs are then linearly combined. 
In this setup, the function \(\hat{f}\) incorporates the FP model of the system along with a trained neural network model, the outputs of the two models are then are then linearly combined. 

Assuming that the system's state variable \(\boldsymbol{x}\) is measurable we can use the observation as ground truth. Given \( N \) observations of the trajectory generated by the real dynamical system sampled at \( \mathbf{T}_{s} = \{t_1, t_2, \dots, t_N\}\), with constant sampling time \(T_{s} \in \mathbb{R}\):
\begin{align*}     
    \boldsymbol{Z} = 
    \begin{bmatrix}
    \boldsymbol{z}^{\top}_1 \\
    \boldsymbol{z}^{\top}_2 \\
    \vdots \\
    \boldsymbol{z}^{\top}_{N-\alpha}
    \end{bmatrix}
    =
    \begin{bmatrix}
    \boldsymbol{x}^{\top}_1 & \boldsymbol{u}^{\top}_1 & \dots & \boldsymbol{u}^{\top}_{1+\alpha} \\
    \boldsymbol{x}^{\top}_2 & \boldsymbol{u}^{\top}_2 & \dots & \boldsymbol{u}^{\top}_{2+\alpha} \\
    \vdots & \vdots & \dots & \\
    \boldsymbol{x}^{\top}_{N-\alpha} & \boldsymbol{u}^{\top}_{N-\alpha} & \dots & \boldsymbol{u}^{\top}_{N}
    \end{bmatrix}
\end{align*}
where $\alpha \in \mathbb{N}^{+}$ is the prediction horizon which will be discussed more in the next section, and \( \boldsymbol{Z} \in \mathbb{R}^{N \times (n+m \alpha)} \) is the collection matrix containing vectors \( \boldsymbol{z}_i \in \mathbb{R}^{(n+m\alpha)} \) containing the observation of the state at time \( t_i \) and the input sequence from time \(t_i\) to time \(t_{i+\alpha}\).

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{images/Resnet.pdf}
%     \caption{Schematic representation of the k-step-ahead prediction with Forward Euler method of the KNODE dynamical model, the FP model \(\tilde{f}\) is integrated into the model \(\hat{f}\) along with the NN $\boldsymbol{\phi}_{\boldsymbol{\theta}}$. The outputs from both the neural network and the knowledge block \(\tilde{f}\) are then linearly coupled. This allows the model to leverage prior knowledge from \(\tilde{f}\) while adapting to the data through the neural network component, ultimately enhancing model performance.}
%     \label{fig:resnet}
% \end{figure}



\subsection{Prediction Error Minimization Problem}


The problem of approximating the residual dynamics can be addressed by minimizing the predictions error of the KNODE model. The residual dynamics of the prediction, that is defined as the prediction error committed by the model, can be evaluated during training and reduced by a NN.

\begin{comment}
Defining the input sequence as follows:
\begin{align*}
    \boldsymbol{u}_k(\boldsymbol{z}_i) = 
    \begin{cases} 
        \boldsymbol{u}_i & \text{if } k=1, \\
        \boldsymbol{u}_{i+1} & \text{if } k=2, \\
        \vdots\\
        \boldsymbol{u}_{i+\alpha} & \text{if } k=\alpha .
    \end{cases}
\end{align*}
We compute the \(k\)-step-ahead prediction, where \(k\) is any positive integer \(k\in \mathbb{N}^+\), integrating the dynamics of the system using forward Euler method:
\begin{align}
    \hat{\boldsymbol{x}}_k( \boldsymbol{z}_i) = \boldsymbol{x}_{i} + \sum_{j=1}^{k} &( \tilde{f}\left(\hat{\boldsymbol{x}}_j( \boldsymbol{z}_i),\boldsymbol{u}_j( \boldsymbol{z}_i) \right) \notag
    \\
    &+ \boldsymbol{\phi}_{\boldsymbol{\theta}}(\hat{\boldsymbol{x}}_j( \boldsymbol{z}_i),\boldsymbol{u}_j( \boldsymbol{z}_i)) ) \, T_{s}
    \label{res-net-prediction}
\end{align}
Comparing the predictions of the hybrid model with the ground truth \(\boldsymbol{x}_i\) we aim to solve a minimization problem where the objective is to minimize the predictions error, and the weights of the NN \(\boldsymbol{\theta}\) are the decision variable of the problem. To accomplish this, we define the mean squared error loss function:
\begin{align*}
    L(\boldsymbol{\theta})= \frac{1}{N-\alpha}\sum_{i = 1}^{N-\alpha} \frac{1}{\alpha} \sum_{k = 1}^{\alpha} \left\|\hat{\boldsymbol{x}}_k(\boldsymbol{z}_i) - \boldsymbol{x}_{k+i}\right\|^2
\end{align*}
where \(\alpha\) is the look-ahead parameter.

The resulting optimization problem that is schematically represented in Fig. \ref{fig:NN_pred} is formulated as follows:
\begin{equation}
    \label{min_residual_opt_problem}
    \min_{\theta} \, L(\theta)
\end{equation}
subject to:
\begin{align*}
    &\hat{\boldsymbol{x}}_k(\boldsymbol{z}_i) = \boldsymbol{x}_i + \sum^{k}_{j=1} \hat{f}(\hat{\boldsymbol{x}}_j, \boldsymbol{u}_j,\boldsymbol{\phi}_{\theta}) T_s \, , \forall t_i \in  \mathbf{T}_{s} \, , \, \forall t_k \in  \mathbf{T}_\alpha \, .
\end{align*}
The constraint defines the hybrid model dynamics  \(\hat{f}\), this constraint ensure that \(\hat{\boldsymbol{x}}\) is a prediction of the hybrid model for every observation at time \(t_i \in \mathbf{T}_{s}\) and for all the predictions in the horizon \(t_k \in \mathbf{T}_\alpha = \{t_{i+1}, \dots , t_{i+\alpha}\} \subset \mathbf{T}_{s}\). 
The parameters \(\boldsymbol{\theta}\) can be estimated by \(\boldsymbol{\boldsymbol{\theta}} = \arg \min_{\theta} L(\boldsymbol{\theta})\).

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/NN_pred.png}
    \caption{A one dimensional example of the ResNet constrained optimization problem. The blue curve is the real time evolution of the system, while the blue dots are the observations, and the red dots are the predictions generated by \(\hat{f}\). In this example \(\alpha\) = 2, and therefore \(\hat{f}\) generates predictions of two sampling time. The loss is then computed as the RMSE between the blue and red dots sampled at every time step.}
    \label{fig:NN_pred}
\end{figure}

   
\subsection{Solving the equality constrained optimization problem}
To solve the optimization problem previously described, we employ the adjoint sensitivity method, which evaluates \(\frac{d L}{d \boldsymbol{\theta}}\) , the sensitivity of the loss function with respect to the parameters \(\boldsymbol{\theta}\).
The adjoint sensitivity method allows the sensitivity to be efficiently computed with constant memory cost over a time interval by evaluating an adjoint variable backwards along the interval. This is a marked contrast with the alternative of backpropagation, which requires one to differentiate through numerical operations and save all of the gradient information. We describe the adjoint sensitivity method and its full derivation in this section.

We consider the subproblem of minimizing the integral \(\int_{t_i}^{t_{i+\alpha}} \delta(t_s - \tau) \left\| \hat{\boldsymbol{x}}(\tau, z(t_i)) - \boldsymbol{x}(\tau) \right\|^2 d\tau\). The full optimization problem is then the sum of \(N-\alpha\) subproblems, namely:
\[
    \min_{\theta} \, F({\boldsymbol{\theta}}) = \int_{t_i}^{t_{i+\alpha}} \delta(t_s - \tau) \left\| \hat{\boldsymbol{x}}(\tau, z(t_i)) - \boldsymbol{x}(\tau) \right\|^2 d\tau
\]
subject to:
\begin{align*} 
    &\dot{\hat{\boldsymbol{x}}}(\tau,\boldsymbol{z}(t_i)) = \hat{f}(\hat{\boldsymbol{x}}(\tau,\boldsymbol{z}(t_i)), \boldsymbol{u}(\boldsymbol{z}(t_i)), \Delta_{\theta}(\hat{\boldsymbol{x}}(\tau,\boldsymbol{z}(t_i)), \boldsymbol{u}(\boldsymbol{z}(t_i)))) \\
    &\hat{\boldsymbol{x}}(t_i, \boldsymbol{z}(t_i)) = \boldsymbol{x}(t_i) 
\end{align*}

First of all we numerically solve \(\dot{\hat{\boldsymbol{x}}}(t)=\hat{f}(\hat{\boldsymbol{x}}(t), \boldsymbol{u}, \Delta_{\boldsymbol{\theta}})\) forward in time from \(t_i\) to \(t_{i+\alpha}\) with the specified initial conditions.
Then we define the Lagrangian function of this problem 
\begin{align*}
    &\mathcal{L}(\hat{\boldsymbol{x}}(t),\boldsymbol{\theta},\boldsymbol{\lambda}) = F(\boldsymbol{\theta}) + \int_{t_i}^{t_{i+\alpha}} \boldsymbol{\lambda}(t)^{\top}\left(\dot{\hat{\boldsymbol{x}}}(t)-\hat{f}(\hat{\boldsymbol{x}}(t), \Delta_{\boldsymbol{\theta}})\right) \, dt
    \\
    &+ \boldsymbol{\mu}(t)^{\top} \left( \hat{\boldsymbol{x}}(t_i) - \boldsymbol{x}(t_i)  \right)
\end{align*}
and derive the adjoint equation, see appendix for more details.
\begin{equation*}
    2 \delta(t_s-t) ( \hat{\boldsymbol{x}}(t)-\boldsymbol{x}(t)) ) - \boldsymbol{\lambda}(t)^{\top} \hat{f}_x - \dot{\boldsymbol{\lambda}}(t)^{\top} = 0
\end{equation*}
where \(\boldsymbol{\lambda}(t)\) is a continuous-time Lagrange multiplier or adjoint variable, and \(\hat{f}_{\hat{\boldsymbol{x}}}\) is the partial derivative of the function \(\hat{f}\) with respect to \(\hat{\boldsymbol{x}}\), evaluated at \(\hat{\boldsymbol{x}} = \hat{\boldsymbol{x}}(t)\). We then numerically solve this equation backward in time with the initial condition \(\boldsymbol{\lambda}(t_{i+\alpha}) = 0\) to obtain the trajectory of \(\boldsymbol{\lambda}(t)\) from \(t = t_{i+\alpha}\) to \(t = t_i\).
Lastly, the sensitivity is given by 
\[
    \frac{d F}{d \boldsymbol{\theta}} = - \int_{t_i}^{t_{i+\alpha}} \boldsymbol{\lambda}(t) \, \hat{f}_{\theta} \, dt,
\]
where \(\hat{f}_{\theta}\) is the partial derivative of \(\hat{f}\) with respect to \(\theta\), evaluated at \(\theta = \theta(t)\). After obtaining this gradient, we can then perform optimization with methods such as gradient descent. Note that \(\hat{f}_{\boldsymbol{x}}\) and \(\hat{f}_{\theta}\) can be efficiently computed with automatic differentiation during the forward pass. 
\end{comment}



% \subsection{Knoledge-Based Neural Ordinary differential Equation (KNODE)}
% ResNets integrate the system dynamics using the forward Euler integration methodology. This methodology when used to integrate system's dynamics introduce additional error and do not guarantee continuity between temporal steps because it relys on the discretized system's dynamics only. 

% To achieve a more accurate representation of the real system, KNODE models the system directly in continuous time and leverages higher-order ODE solvers to integrate its dynamics.

% KNODE can be seen as a generalization of ResNets. The key distinction between KNODE and ResNets lies in the type of solver employed to integrate the dynamics during model prediction. Specifically, ResNets can be interpreted as a special case of KNODE where the Forward Euler method is used for integration and to compute the model's predictions.

% Comparing the schematic representation of the prediction error minimization problem of ResNets in Fig. \ref{fig:NN_pred} and KNODE in Fig. \ref{fig:KNODE_pred}, using higher-order solvers to integrate system dynamics leads to more precise predictions compared to the Forward Euler method. This improvement is due to the enhanced continuity between successive steps, as higher-order solvers interpolate additional samples within the time step \(T_s\). Consequently, the resulting trajectory is more accurate, especially for extended prediction horizons \(\mathbf{T}_\alpha\).

% In the following part of this section we show an adaptation of the work in \cite{jiahao_knowledge-based_2021} that includes the control input of the system and formulates the same problem shown in the previous section in a continuous time domain.
% \subsection{Prediction error minimization problem}

Differently from the work proposed by \cite{jiahao_knowledge-based_2021} in which KNODE is used to learn autonomous systems, in this work we extend the usage of KNODE to controlled systems, i.e. the inputs of the NN are not solely the states of the system \(\boldsymbol{x}(t)\) but also exogenous variables \(\boldsymbol{u}(t)\) that in general do not depend on the model's state.

In this work, we assume that \(\boldsymbol{u}(t)\) is known. However, this assumption does not generally hold in practical scenarios. In many applications, the inputs to a system are not explicitly modeled, meaning that we lack a closed-form expression for \(\boldsymbol{u}(t)\). Instead, these inputs must either be measured directly or approximated.

% For instance, in MRAV systems the input \(\boldsymbol{u}(t)\) consists of two components: the rotors thrusts vector \(\boldsymbol{\gamma}\) and the external wrench \(\boldsymbol{w}_{e}\). The rotors thrusts vector \(\boldsymbol{\gamma}\) is a digital signal computed by the controller and can be directly evaluated. Conversely, the external wrench \(\boldsymbol{w}_{e}\) represents a physical quantity that cannot be fully captured by analytical models because of its randomness.
For instance, in MRAV systems the input \(\boldsymbol{u}(t)\) consists of the rotors thrusts vector \(\boldsymbol{\gamma}\). The rotors thrusts vector \(\boldsymbol{\gamma}\) can be approximated using a thrust model and the estimated rotors' rotational velocity. The input sequence can be approximated to be constant within a sampling time. 
% \begin{align*}
%     \boldsymbol{u}(t,\boldsymbol{z}_i) = \boldsymbol{u}(t_i+t)
% \end{align*}
\begin{align*}
\boldsymbol{u}(t, \boldsymbol{z}_i) =
\begin{cases} 
    \boldsymbol{u}_i, & \text{if } t \in [t_i, t_{i+1}], \\ 
    \boldsymbol{u}_{i + 1}, & \text{if } t \in [t_{i+1}, t_{i+2}], \\ 
\vdots & \\
    \boldsymbol{u}_{i + \alpha -1}, & \text{if }  t \in [t_{i+\alpha-1}, t_{i+\alpha}].
\end{cases}
% }
\end{align*}

\begin{comment} 
    \boldsymbol{u}_i & \text{if } t_i < t \leq t_{i+1}, \\
    \boldsymbol{u}_{i+1} & \text{if } t_{i+1} < t \leq t_{i+2}, \\
    \vdots\\
    \boldsymbol{u}_{i+\alpha} & \text{if } t_{i+\alpha-1} < t \leq t_{i+\alpha}.
\end{comment}

% \textcolor{green}{}
% In order to evaluate the prediction error, we compute the KNODE model dynamics by integrating it on a specific interval of time:
% \begin{align}
%     \hat{\boldsymbol{x}}(t, \boldsymbol{z}_i) = \boldsymbol{x}_{i} + \int_{t_i}^{t} &( \tilde{f}\left(\hat{\boldsymbol{x}}(\tau, \boldsymbol{z}_i),\boldsymbol{u}(\tau, \boldsymbol{z}_i) \right) \notag
%     \\
%     &+ \boldsymbol{\phi}_{\boldsymbol{\theta}}(\hat{\boldsymbol{x}}(\tau, \boldsymbol{z}_i),\boldsymbol{u}(\tau, \boldsymbol{z}_i)) ) \, d\tau
%     \label{node-prediction}
% \end{align}

In order to evaluate the prediction error, we compute the KNODE model prediction by integrating the KNODE dynamics on a specific interval of time, using an \texttt{ODEsolver}:
\begin{align}
    \hat{\boldsymbol{x}}(t, \boldsymbol{z}_i) = \boldsymbol{x}_{i} + \int_{t_i}^{t} &( \tilde{f}\left(\hat{\boldsymbol{x}}(\tau, \boldsymbol{z}_i),\boldsymbol{u}(\tau, \boldsymbol{z}_i) \right) \notag
    \\
    &+ \boldsymbol{\phi}_{\boldsymbol{\theta}}(\hat{\boldsymbol{x}}(\tau, \boldsymbol{z}_i),\boldsymbol{u}(\tau, \boldsymbol{z}_i)) ) \, d\tau
    \label{node-prediction}
\end{align}

Comparing the predictions of the KNODE model with the ground truth \(\boldsymbol{x}_i\), we formulate an optimization problem where the objective is to minimize the predictions error, with the weights of the NN, \(\boldsymbol{\theta}\), as the decision variable of the problem. Therefore, the mean squared error loss function is defined as:
% To describe the loss function define in \eqref{min_residual_opt_problem} in continuous time we use the dirac delta function \(\delta\):
\begin{align}
    L(\boldsymbol{\theta}) =& \frac{1}{N-\alpha}\sum_{i = 1}^{N-\alpha}
    \notag \\
    &\frac{1}{\alpha} \int_{t_i}^{t_{i+\alpha}} \delta(t_s-\tau)\left\|\hat{\boldsymbol{x}}(\tau,\boldsymbol{z}_i) - \boldsymbol{x}_{k+i}\right\|^2 \, d\tau
    \label{eq-loss}
\end{align}
where \(t_s\) is every time step in \(\mathbf{T}_s\) and \(\delta\) is the dirac delta function.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/KNODE_scheme.pdf}
    \caption{A one dimensional example of the KNODE constrained optimization problem. The blue curve is the real time evolution of the system, while the blue dots are the observations, and the red curves are the predictions generated by \(\hat{f}\) and the red dots are the samling at \(t_s \in \mathbf{T}_s\). In this example \(\alpha\) = 2, and therefore \(\hat{f}\) generates predictions of two sampling time. The loss is then computed as the RMSE between the blue and red dots sampled at every time step in \(\mathbf{T}_s\).}
    \label{fig:KNODE_pred}
\end{figure}

The resulting optimization problem, depicted in Fig. \ref{fig:KNODE_pred} is formulated as follows:
\begin{subequations}
    \label{KNODE_min_residual_opt_problem}
\begin{align}
    \min_{\theta} \, &L(\theta) 
    \\
    \text{s.t.}: \notag
    \\ 
    &\hat{\boldsymbol{x}}(t,\boldsymbol{z}_i) = \boldsymbol{x}_i + \int^{t}_{t_{i}} \hat{f}(\hat{\boldsymbol{x}}, \boldsymbol{u},\boldsymbol{\phi}_{\theta}) \, d\tau , \notag
    \\
    &\qquad \qquad \qquad \quad \forall t_i \in  \mathbf{T}_{s} \, , \, \forall t \in \mathbf{T}_\alpha
    \\
    &\hat{\boldsymbol{x}}(0,\boldsymbol{z}_i) = \boldsymbol{x}_i, \quad \forall t_i \in  \mathbf{T}_{s}
\end{align}
\end{subequations}

where \(\mathbf{T}_\alpha = [t_i,t_{i+\alpha}]\).

The constraints define the KNODE model dynamics  \(\hat{f}\), this constraints ensure that \(\hat{\boldsymbol{x}}\) is a prediction of the KNODE model for every observation at time \(t_i \in \mathbf{T}_{s}\) and for all the predictions in the horizon \(t_k \in \mathbf{T}_\alpha = \{t_{i+1}, \dots , t_{i+\alpha}\} \subset \mathbf{T}_{s}\). 

The NN parameters \(\boldsymbol{\theta}\) can be estimated by 
\begin{equation}
    \boldsymbol{\boldsymbol{\theta}} = \arg \min_{\theta} \quad L(\boldsymbol{\theta})
\end{equation}

% \textcolor{red}{Explain what $\alpha$ is and how if effects the learning and predictions.}

% \textcolor{green}{THIS IS A COPY AND PASTE FROM THE KNODE PAPER In some cases a larger lookahead makes the learning more robust to noise. This may be due to the fact that a small lookahead overfits to noise more easily. In addition, using a larger lookahead gives more overlaps between predicted trajectories, and therefore encourages smoothness and reduces the e effect of noises. But if the training solver incurs significant numerical errors at every step, the lookahead should be small. Large numerical error happens if the numerical integration scheme uses very large steps or is of low order such as the forward Euler method adopted in the proposed observer scheme. Since a larger lookahead means more numerical integration steps, the numerical errors can propagate through the trajectory and get amplified, rendering the resulting loss inaccurate.}

In this problem, the prediction horizon parameter, $\alpha$, plays an important role is determining the performance and generalizability of the learned model. As discussed in \cite{jiahao_knowledge-based_2021}, increasing $\alpha$ can make the model robust against noise, and also it reduces the sensitivity of the model leading to smoother predictions. Hoever, higher $\alpha$ also means more numerical integration steps, which means more computationally heavy model and the possibility of increased accumulated numerical errors.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.66\linewidth]{images/Knode.pdf}
%     \caption{Schematic representation of the k-step-ahead prediction with higher order integration methods of the KNODE model. In contrast to \ref{fig:resnet} this scheme interpolate  additional samples within the time step \(T_s\). Consequently, the resulting trajectory is more accurate The scheme is initialized passing the collection vector \(\boldsymbol{z}_i\) containing the initial state \(\boldsymbol{x}_i\) at time \(t_i\) and the input sequance defined in continuous time \(\boldsymbol{u}(\tau,\boldsymbol{z}_i)\)}
%     \label{fig:Knode}
% \end{figure}


% \subsection{Training KNODE Model}
% In this section we provide a detailed description of the training pipeline for KNODE on MRAV systems.
% In our framework the state \(\boldsymbol{x}\) is the twist of the body \(\twist\) while the input is the rotors thrusts vector defined by the controller \(\boldsymbol{\gamma}\) and the measured external wrench \( \boldsymbol{w}_{e} \) applied to the body, namely 
% \begin{equation}
%     \boldsymbol{u}= \begin{bmatrix}
%         \boldsymbol{\gamma}^{\top}  & \boldsymbol{w}_{e}^{\top} \
%     \end{bmatrix}^{\top}
% \end{equation}
% The known dynamics of the system have already been defined in \eqref{eq-euler-lagrange} and can be rewritten using the same notation of \eqref{partial_knowledge}:
% \begin{equation*}
%     \tilde{f}(\twist,\boldsymbol{u}) = \dtwist = \mathbf{M}^{-1} \left( - \boldsymbol{h} (\twist) + \mathbf{G} \boldsymbol{\gamma} + \boldsymbol{w}_{e} \right)
% \end{equation*}

% In our framework the KNODE model defined in \eqref{eq-f-hat-KNODE}, including both the known dynamics of the system and the NN is defined as follows:
% \begin{align}
%     \dot{\hat{\twist}}_B = \hat{f}(\hat{\twist}_B,\boldsymbol{u}) = \tilde{f}(\hat{\twist}_B,\boldsymbol{u}) + \boldsymbol{\phi}_{\boldsymbol{\theta}}(\hat{\twist}_B, \boldsymbol{u})
%     \label{KNODE_MRAV}
% \end{align}
% Where \(\boldsymbol{\phi}_{\boldsymbol{\theta}}\) is a neural network that parameterize the unknown residual dynamics \(\boldsymbol{\phi}\).
% \[\boldsymbol{\phi}_{\boldsymbol{\theta}}:\mathbb{R}^n\times\mathbb{R}^m\rightarrow\mathbb{R}^n
% \]
% where, \(m\) is the dimension of the input vector \(\boldsymbol{u}\).

% \begin{comment}
% The collected data, ideally obtained by fusing optitrack and IMU sensor data to accurately estimate the twist \(\twist\) ahe force torque sensor is needed to measure the interaction forces, the external wrench \(\boldsymbol{w}_{e}\) is then computed knowing the geometrical properties of the position of the force torque sensor with respect the CoM. Both these quantities are sampled at \( 1 KHz \) filtered and down-sampled at the controller frequency? (this is just an idea on how I would do it), the thrust input is provided by the designed controller.
% \end{comment}
% The collection matrix consists of the twist \(\twist_{B,i}\), external wrench \(\boldsymbol{w}_{e,i}\) and the controller input thrusts \(\boldsymbol{\gamma}_i\), sampled at every time \(t_i\):

% \begin{align}   
%     \label{Collection_martrix}
%     \boldsymbol{Z} = 
%     \begin{bmatrix}
%     \boldsymbol{z}^{\top}_1 \\
%     \boldsymbol{z}^{\top}_2 \\
%     \vdots \\
%     \boldsymbol{z}^{\top}_{N-\alpha}
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%     \twist^{\top}_{B,1} & \boldsymbol{u}^{\top}_1 & \dots & \boldsymbol{u}^{\top}_{1+\alpha} \\
%     \twist^{\top}_{B,2} & \boldsymbol{u}^{\top}_2 & \dots & \boldsymbol{u}^{\top}_{2+\alpha} \\
%     \vdots & \vdots & \dots & \\
%     \twist^{\top}_{B,N-\alpha} & \boldsymbol{u}^{\top}_{N-\alpha} & \dots & \boldsymbol{u}^{\top}_{N}
%     \end{bmatrix}
% \end{align}
% Where, \(\boldsymbol{u}_i = [\boldsymbol{\gamma}_i^\top,\boldsymbol{w}_{e,i}^\top]^\top\) are the collected input thrust of the controller and the measured wrench at time \(t_i\).

% \begin{comment}
% To solve the prediction error minimization problem described in \eqref{min_residual_opt_problem}, we start by computing the \(k\)-step-ahead prediction for each \(t_i \in \mathbf{T}_s\) in a prediction horizon of samples \(t_k \in \mathbf{T}_\alpha\) defined by the look-ahead \(\alpha\), namely:
% \begin{align*}
%     \hat{\twist}_{k}(\boldsymbol{z}_i) = \twist_{B,i} + \sum^{k}_{j=1} \hat{f}(\hat{\twist}_{j}, \boldsymbol{u}_j,\boldsymbol{\phi}_{\theta}) T_s
% \end{align*}
% Note that the constraints of \eqref{min_residual_opt_problem} are satisfied by construction.
% After computing the predictions we evaluate the prediction error, thus the loss function can be computed as follows:
% \begin{align}
%     L(\boldsymbol{\theta})= \frac{1}{N-\alpha}\sum_{i = 1}^{N-\alpha} \frac{1}{\alpha} \sum_{k = 1}^{\alpha} \left\| \hat{\twist}_{k}( \boldsymbol{z}_i) - \twist_{B,k+i} \right\|^2
%     \label{loss}
% \end{align}
% \end{comment}

% To solve the optimization problem described in \eqref{KNODE_min_residual_opt_problem}, we employed the Adam optimizer \cite{kingma_adam_2017}, a method known for its efficiency in handling stochastic and non-stationary loss functions. The loss function defined in \eqref{eq-loss} is stochastic as it consists of a sum of predictions evaluated over various samples of noisy data. In this context, the Adam algorithm enhances optimization efficiency by effectively adapting learning rates and managing gradient updates.

% \begin{comment}
% When training a neural network, we aim to adjust its weights, \(\boldsymbol{\theta}\), to minimize the loss function \(L(\boldsymbol{\theta})\). 

%     Ideally, a perfect model would achieve zero loss for all inputs, but in practical scenarios, the goal is to iteratively refine the weights until the loss is tolerable and the model generalizes well to unseen data.

% The key question we address is: how do we determine the direction and magnitude of weight updates? In other words, how can we compute the gradients of the loss function with respect to the model's weights, \(\frac{\partial L}{\partial \boldsymbol{\theta}}\)?

% As networks grow deeper and more complex, symbolic computation of these gradients becomes impractical due to the big number of operations involved. PyTorch’s \texttt{autograd} \cite{paszke_automatic_nodate} module automates this process efficiently through two key steps:

% \begin{itemize}
%     \item Forward Pass: During the forward pass, \texttt{autograd} builds a computation graph by tracking all operations and their intermediate results. For each operation, it stores the local gradients of the output with respect to its inputs. This graph represents how each parameter in the model contributes to the output.
    
%     \item Backpropagation of the gradients: when calling the backpropagation method, \texttt{autograd} applies the chain rule to compute the gradients of the loss function with respect to the weights. It traverses the computation graph in reverse for every generated output, combining local gradients to calculate \(\frac{\partial L}{\partial \boldsymbol{\theta}}\) for all parameters efficiently.
% \end{itemize}
% \end{comment}
% In Alg. \ref{alg:nn_training} we summarize the training pipeline of KNODE. It is important to notice that differently from \cite{chen_neural_2018} and \cite{jiahao_knowledge-based_2021} in this work we do not solve the co-state equation using the Adjoint Sensitivity method.
% \begin{algorithm}
% \caption{Training pipeline of KNODE}
% \label{alg:nn_training}
% \begin{algorithmic}[1]
% \REQUIRE Dataset \( \mathbf{Z} \), prediction horizon \( \alpha \)
% \ENSURE Trained weights \( \boldsymbol{\theta} \)
% \STATE Initialize weights \( \boldsymbol{\theta} \)
% \WHILE{stopping criteria not met}
%     \FOR{\( i \) in \(\mathbf{T}_s \)}
%         \FOR{\( k \) in \( \mathbf{T}_\alpha \)}
%             \STATE Compute predictions \(\hat{\twist}_{k}\) using current \( \boldsymbol{\theta} \).
%             \STATE Compute the RMSE of prediction.
%             \STATE Update the Loss \(L(\boldsymbol{\theta}) \).
%         \ENDFOR
%     \ENDFOR
%     \STATE Back-propagate the gradients \(\frac{\partial L}{\partial \boldsymbol{\theta}}\).
%     \STATE Update weights using Adam.
% \ENDWHILE
% \RETURN \( \boldsymbol{\theta} \)
% \end{algorithmic}
% \end{algorithm}

% After tuning the parameters $\boldsymbol{\theta}$ of the NN $\boldsymbol{\phi}_\theta$ through the NN training, the NN $\boldsymbol{\phi}_\theta$ will learn to captures the residual dynamics $\boldsymbol{\phi}$. Therefore, the KNODE model $\hat{f}(\hat{\boldsymbol{x}},\boldsymbol{u},\boldsymbol{\phi}_{\theta}(\hat{\boldsymbol{x}},\boldsymbol{u}))$ will approximate the real dynamics of the system $f\left(\boldsymbol{x},\boldsymbol{u}\right)$

% \begin{align*}
%     \boldsymbol{\phi}_\theta &\approx \boldsymbol{\phi} \\
%     \quad \hat{f} \left(\hat{\boldsymbol{x}},\boldsymbol{u},\boldsymbol{\phi}_{\theta}\left(\hat{\boldsymbol{x}},\boldsymbol{u}\right)\right) &\approx f\left(\boldsymbol{x},\boldsymbol{u}\right)
% \end{align*}

\subsection{Training KNODE Model}
In this section we provide a detailed description of the training pipeline for KNODE on MRAV systems. 

Since we want to use the KNODE model for wrench estimation, we will assume that the training dataset is generated by a system that had no external wrench applied to it, this means that the system dynamics to be learned is written as:
\begin{equation}
    f\left(\boldsymbol{x},\boldsymbol{u}\right) = \mathbf{M}^{-1} \left(
    - \boldsymbol{h} (\twist)  +
    \boldsymbol{w}_{a} \right) + \boldsymbol{\phi}
\end{equation}
notice the absence of the external wrench $\boldsymbol{w}_e$.


This assumption will allow the KNODE model to learn the residual dynamics without requiring any external wrench measurements, but more importantly, it will allow us to use the learned KNODE model in a classical wrench observer such as the momentum-based observer described in section \ref{sec-momentum-SOTA}. 

 % \textcolor{green}{}

This means that when there is no external wrench applied to the system, the trained KNODE model predictions will be "almost perfect", while when there is an external wrench, the KNODE model predictions will be different from the real measurements which will allow the wrench observer that uses the KNODE model to estimate the external wrench. 
% \textcolor{green}{}

% In our framework the state \(\boldsymbol{x}\) is the twist of the body \(\twist\) while the input is the rotors thrusts vector defined by the controller \(\boldsymbol{\gamma}\), namely 
% \begin{equation}
%     \boldsymbol{x} \coloneq 
%         \twist
%     , 
%     \quad
%     \boldsymbol{u} \coloneq
%         \boldsymbol{\gamma}
% \end{equation}
\begin{comment}

The known dynamics of the system have already been defined in \eqref{eq-euler-lagrange} and can be rewritten using the same notation of \eqref{partial_knowledge}:
\begin{equation*}
    \tilde{f}(\twist,\boldsymbol{u}) = \dtwist = \mathbf{M}^{-1} \left( - \boldsymbol{h} (\twist) + \mathbf{G} \boldsymbol{\gamma} \right)
\end{equation*}
Note that in the equation above, the external wrench $\boldsymbol{w}_e$ is absent.

In our framework the KNODE model defined in \eqref{eq-f-hat-KNODE}, including both the known dynamics of the system and the NN is defined as follows:
\begin{align}
    \dot{\hat{\twist}}_B = \hat{f}(\hat{\twist}_B,\boldsymbol{u}) = \tilde{f}(\hat{\twist}_B,\boldsymbol{u}) + \boldsymbol{\phi}_{\boldsymbol{\theta}}(\hat{\twist}_B, \boldsymbol{u})
    \label{KNODE_MRAV}
\end{align}

Where $\boldsymbol{\phi}_{\boldsymbol{\theta}}:\mathbb{R}^n\times\mathbb{R}^m\rightarrow\mathbb{R}^n$ is a neural network that parameterize the unknown residual dynamics \(\boldsymbol{\phi}\),  and \(m\) is the dimension of the input vector \(\boldsymbol{u}\).

The collected data, ideally obtained by fusing optitrack and IMU sensor data to accurately estimate the twist \(\twist\) ahe force torque sensor is needed to measure the interaction forces, the external wrench \(\boldsymbol{w}_{e}\) is then computed knowing the geometrical properties of the position of the force torque sensor with respect the CoM. Both these quantities are sampled at \( 1 KHz \) filtered and down-sampled at the controller frequency? (this is just an idea on how I would do it), the thrust input is provided by the designed controller.
The collection matrix consists of the twist \(\twist_{B,i}\) and the controller input thrusts \(\boldsymbol{\gamma}_i\), sampled at every time \(t_i\) \textcolor{red}{Add more details about why we need future $\gamma$}:

\begin{align}   
    \label{Collection_martrix}
    \boldsymbol{Z} = 
    \begin{bmatrix}
    \boldsymbol{z}^{\top}_1 \\
    \boldsymbol{z}^{\top}_2 \\
    \vdots \\
    \boldsymbol{z}^{\top}_{N-\alpha}
    \end{bmatrix}
    =
    \begin{bmatrix}
    \twist^{\top}_{B,1} & \boldsymbol{\gamma}^{\top}_1 & \dots & \boldsymbol{\gamma}^{\top}_{1+\alpha} \\
    \twist^{\top}_{B,2} & \boldsymbol{\gamma}^{\top}_2 & \dots & \boldsymbol{\gamma}^{\top}_{2+\alpha} \\
    \vdots & \vdots & \dots & \\
    \twist^{\top}_{B,N-\alpha} & \boldsymbol{\gamma}^{\top}_{N-\alpha} & \dots & \boldsymbol{\gamma}^{\top}_{N}
    \end{bmatrix}
\end{align}
% Where, \(\boldsymbol{u}_i = [\boldsymbol{\gamma}_i^\top,\boldsymbol{w}_{e,i}^\top]^\top\) are the collected input thrust of the controller and the measured wrench at time \(t_i\).

To solve the prediction error minimization problem described in \eqref{min_residual_opt_problem}, we start by computing the \(k\)-step-ahead prediction for each \(t_i \in \mathbf{T}_s\) in a prediction horizon of samples \(t_k \in \mathbf{T}_\alpha\) defined by the look-ahead \(\alpha\), namely:
\begin{align*}
    \hat{\twist}_{k}(\boldsymbol{z}_i) = \twist_{B,i} + \sum^{k}_{j=1} \hat{f}(\hat{\twist}_{j}, \boldsymbol{u}_j,\boldsymbol{\phi}_{\theta}) T_s
\end{align*}
Note that the constraints of \eqref{min_residual_opt_problem} are satisfied by construction.
After computing the predictions we evaluate the prediction error, thus the loss function can be computed as follows:
\begin{align}
    L(\boldsymbol{\theta})= \frac{1}{N-\alpha}\sum_{i = 1}^{N-\alpha} \frac{1}{\alpha} \sum_{k = 1}^{\alpha} \left\| \hat{\twist}_{k}( \boldsymbol{z}_i) - \twist_{B,k+i} \right\|^2
    \label{loss}
\end{align}
\end{comment}

To solve the optimization problem described in \eqref{KNODE_min_residual_opt_problem}, we employed the Adam optimizer \cite{kingma_adam_2017}, a method known for its efficiency in handling stochastic and non-stationary loss functions. The loss function defined in \eqref{eq-loss} is stochastic as it consists of a sum of predictions evaluated over various samples of (possibly) noisy data. 

\begin{comment}
When training a neural network, we aim to adjust its weights, \(\boldsymbol{\theta}\), to minimize the loss function \(L(\boldsymbol{\theta})\). 

    Ideally, a perfect model would achieve zero loss for all inputs, but in practical scenarios, the goal is to iteratively refine the weights until the loss is tolerable and the model generalizes well to unseen data.

The key question we address is: how do we determine the direction and magnitude of weight updates? In other words, how can we compute the gradients of the loss function with respect to the model's weights, \(\frac{\partial L}{\partial \boldsymbol{\theta}}\)?

As networks grow deeper and more complex, symbolic computation of these gradients becomes impractical due to the big number of operations involved. PyTorch’s \texttt{autograd} \cite{paszke_automatic_nodate} module automates this process efficiently through two key steps:

\begin{itemize}
    \item Forward Pass: During the forward pass, \texttt{autograd} builds a computation graph by tracking all operations and their intermediate results. For each operation, it stores the local gradients of the output with respect to its inputs. This graph represents how each parameter in the model contributes to the output.
    
    \item Backpropagation of the gradients: when calling the backpropagation method, \texttt{autograd} applies the chain rule to compute the gradients of the loss function with respect to the weights. It traverses the computation graph in reverse for every generated output, combining local gradients to calculate \(\frac{\partial L}{\partial \boldsymbol{\theta}}\) for all parameters efficiently.
\end{itemize}
\end{comment}
In Alg. \ref{alg:nn_training} we summarize the training pipeline of KNODE. It is important to notice that differently from \cite{chen_neural_2018} and \cite{jiahao_knowledge-based_2021} in this work we do not solve the co-state equation using the Adjoint Sensitivity method.
\begin{algorithm}
\caption{Training pipeline of KNODE}
\label{alg:nn_training}
\begin{algorithmic}[1]
\REQUIRE Dataset \( \mathbf{Z} \), prediction horizon \( \alpha \)
\ENSURE Trained weights \( \boldsymbol{\theta} \)
\STATE Initialize weights \( \boldsymbol{\theta} \)
\WHILE{stopping criteria not met}
    \FOR{\( i \) in \(\mathbf{T}_s \)}
        \FOR{\( k \) in \( \mathbf{T}_\alpha \)}
            \STATE Compute predictions \(\hat{\twist}_{k}\) using current \( \boldsymbol{\theta} \).
            \STATE Compute the RMSE of prediction.
            \STATE Update the Loss \(L(\boldsymbol{\theta}) \).
        \ENDFOR
    \ENDFOR
    \STATE Back-propagate the gradients \(\frac{\partial L}{\partial \boldsymbol{\theta}}\).
    \STATE Update weights using Adam.
\ENDWHILE
\RETURN \( \boldsymbol{\theta} \)
\end{algorithmic}
\end{algorithm}

After tuning the parameters $\boldsymbol{\theta}$ of the NN $\boldsymbol{\phi}_\theta$ through the NN training, the NN $\boldsymbol{\phi}_\theta$ will learn to captures the residual dynamics $\boldsymbol{\phi}$. Therefore, the KNODE model $\hat{f}(\hat{\boldsymbol{x}},\boldsymbol{u},\boldsymbol{\phi}_{\theta}(\hat{\boldsymbol{x}},\boldsymbol{u}))$ will approximate the real dynamics of the system $f\left(\boldsymbol{x},\boldsymbol{u}\right)$ in the absence of external wrench $\boldsymbol{w}_e$, such that:

\begin{align*}
    \boldsymbol{\phi}_\theta &\approx \boldsymbol{\phi} \\
    \quad \hat{f} \left(\hat{\boldsymbol{x}},\boldsymbol{u},\boldsymbol{\phi}_{\theta}\left(\hat{\boldsymbol{x}},\boldsymbol{u}\right)\right) &\approx f\left(\boldsymbol{x},\boldsymbol{u}\right)
\end{align*}

==> old_things/old_tables.tex <==
\begin{table}[b]
\centering
\caption{Model Mismatch Type and the Parameters Errors}
% \vspace{-3 mm}
% {Here}
% \vspace{2 mm}
% \\
\begin{tabular}{l c c c c c c}
\toprule
 & \multicolumn{6}{c@{}}{\textbf{Model Mismatch Type}} \\ 
\cmidrule(l){2-7}
\textbf{Parameter}        & \textbf{M} & \textbf{G} & \textbf{MG-1} & \textbf{MG-2} & \textbf{D} & \textbf{MGD} \\
\midrule
Mass                   & -2.5 \%                       &                  & -2.5 \%                  & -2.5 \%  & 0 \%    & -2.5 \%              \\
Inertia         & 3.5 \%                        &                & 3.5 \%                   & 3.5 \%          & 0 \%     & 3.5 \%    \\
Rotors Model:      & & & &                  \\ 

\quad Tilt angle                  &                          & 10 \%                & 5 \%                   & 10 \%  & 0 \%     & 5 \%             \\ 
\quad Arm length                      &                          & -5 \%                & -2.5 \%                  & -5 \%    & 0 \%   & -2.5 \%           \\ 
\quad $c_d$                   &                          & -40 \%               & -20 \%                 & -40 \%            & 0 \%    & -20 \%  \\ 
\quad $c_f$                   &                          & 40 \%                & 20 \%                  & 40 \%            & 0 \%    & 20 \%   \\ 

$d_1, d_2 = $ & & & & & 0.1 & 0.1 \\
\bottomrule
\end{tabular}
\label{tab-uncertainity}
\end{table}

\begin{table*}[ht]
\centering
\caption{RMSE Comparison Table}
\begin{tabular}{l l l >{$}c<{$} >{$}c<{$} >{$}c<{$} >{$}c<{$} >{$}c<{$}}
\toprule
&  & \textbf{Observer} & \multicolumn{4}{c@{}}{\textbf{Flying Scenario}} & \\ 
\cmidrule(l){4-7}
& \textbf{}        &  & \textbf{Hovering} & \textbf{Free Flight} & \textbf{Hov.+Ext.Wr.} & \textbf{FF+Ext.Wr.} & \textbf{All} \\ 
\cmidrule(l){2-8}
\multirow{24}{*}{\rotatebox[origin=c]{90}{\textbf{Model Mismatch Type}}} & \multirow{4}{*}{\textbf{M}}     & MO   & \textbf{0.4906}       & 3.8998       & \textbf{2.3262}       & 6.9415       & 13.6581         \\ 
&                                 & NeMO, $\alpha = 1$        & 0.6126       & 2.8444       & 2.7947       & 5.3986       & 11.6502         \\ 
&                                 & NeMO, $\alpha = 10$        & 0.6127       & 2.0803       & 2.7325       & 4.8749       & 10.3004         \\ 
&                                 & NeMO, $\alpha = 50$        & 0.6129       & \textbf{2.0454}       & 2.7303       & \textbf{4.8263}       & \textbf{10.2149}         \\ 
\cmidrule(l){2-8}
& \multirow{4}{*}{\textbf{G}}      & MO   & \textbf{0.4989}       & 10.4734      & 4.7469       & 13.3873      & 29.1066          \\ 
&                             & NeMO, $\alpha = 1$          & 0.6119            & 2.5400               & 2.7268                & 5.2476              & 11.1263         \\ 
&                             & NeMO, $\alpha = 10$         & 0.6125            & 1.9511               & \textbf{2.7168}                & 4.7016              & 9.9821          \\ 
&                             & NeMO, $\alpha = 50$         & 0.6117            & \textbf{1.9188}               & 2.7226                & \textbf{4.5731}              & \textbf{9.8262}          \\ 
\cmidrule(l){2-8}
& \multirow{4}{*}{\textbf{MG-1}}     & MO   & \textbf{0.4929}       & 7.7544       & 3.3246       & 10.6532      & 22.2251         \\ 
&                             &NeMO, $\alpha = 1$       & 0.6134            & 2.7401               & 2.7606                & 5.7572              & 11.8713         \\ 
&                                 & NeMO, $\alpha = 10$       & 0.6127            & 2.1461               & \textbf{2.7283}                & 4.9880              & 10.4751         \\ 
&                                 & NeMO, $\alpha = 50$       & 0.6129            & \textbf{2.0078}               & 2.7286                & \textbf{4.8814}              & \textbf{10.2307 }        \\ 
\cmidrule(l){2-8}
& \multirow{4}{*}{\textbf{MG-2}}      & MO   & \textbf{0.4989}       & 12.2648      & 4.7484       & 15.9152      & 33.4273         \\ 
&                             & NeMO, $\alpha = 1$       & 0.6155            & 2.5696               & 2.8015                & 5.0190              & 11.0057         \\ 
&                                 & NeMO, $\alpha = 10$      & 0.6139            & 2.1411               & 2.7531                & 4.8689              & 10.3769         \\ 
&                                 & NeMO, $\alpha = 50$      & 0.6136            & \textbf{2.0096}               & \textbf{2.7364}                & \textbf{4.7566}              & \textbf{10.1161}         \\ 
\cmidrule(l){2-8}
& \multirow{4}{*}{\textbf{D}}       & MO   & \textbf{0.4906}       & \textbf{1.5187}       & \textbf{2.3244}       & \textbf{4.0709}       & \textbf{8.4046}         \\ 
&                                   & NeMO, $\alpha = 1$      & 0.6127       & 2.1672       & 2.7420       & 5.0142       & 10.5362         \\ 
&                                   & NeMO, $\alpha = 10$     & 0.6125       & 2.1132       & 2.7269       & 4.8429       & 10.2954         \\ 
&                                   & NeMO, $\alpha = 50$     & 0.6119       & 1.9402       & 2.7240       & 4.7739       & 10.0500         \\ 
\cmidrule(l){2-8}
& \multirow{4}{*}{\textbf{MGD}}         & MO   & \textbf{0.4929}       & 7.2539       & 3.0301       & 10.5231      & 21.3000         \\ 
&                                       & NeMO, $\alpha = 1$      & 0.6150       & 2.6343       & 2.7527       & 5.3314       & 11.3334         \\ 
&                                       & NeMO, $\alpha = 10$     & 0.6145       & 2.0506       & 2.7376       & 4.9657       & 10.3683         \\ 
&                                       & NeMO, $\alpha = 50$     & 0.6143       & \textbf{1.9662}       & \textbf{2.7336}       & \textbf{4.8956}       & \textbf{10.2097}         \\ 
\bottomrule
\end{tabular}
\label{tab:rmse_error}
\end{table*}

% \begin{table*}[ht]
% \centering
% \caption{RMSE Comparison Table}
% \begin{tabular}{l l >{$}c<{$} >{$}c<{$} >{$}c<{$} >{$}c<{$} >{$}c<{$}}
% \toprule

%  & & \multicolumn{4}{c@{}}{\textbf{Flying Scenario}} & \\ 
% \cmidrule(l){3-6} \\

% \textbf{}        &  & \textbf{Hovering} & \textbf{Free Flight} & \textbf{Hov.+Ext.Wr.} & \textbf{FF+Ext.Wr.} & \textbf{All} \\ 

% \midrule

% \multirow{4}{*}{\textbf{M}}     & MO   & \textbf{0.4906}       & 3.8998       & \textbf{2.3262}       & 6.9415       & 13.6581         \\ 
%                                 & \alpha = 1        & 0.6126       & 2.8444       & 2.7947       & 5.3986       & 11.6502         \\ 
%                                 & \alpha = 10        & 0.6127       & 2.0803       & 2.7325       & 4.8749       & 10.3004         \\ 
%                                 & \alpha = 50        & 0.6129       & \textbf{2.0454}       & 2.7303       & \textbf{4.8263}       & \textbf{10.2149}         \\ 

% \midrule

% \multirow{3}{*}{\textbf{G}}      & MO   & \textbf{0.4989}       & 10.4734      & 4.7469       & 13.3873      & 29.1066          \\ 
%                             & \alpha = 1          & 0.6119            & 2.5400               & 2.7268                & 5.2476              & 11.1263         \\ 
%                             & \alpha = 10         & 0.6125            & 1.9511               & \textbf{2.7168}                & 4.7016              & 9.9821          \\ 
%                             & \alpha = 50         & 0.6117            & \textbf{1.9188}               & 2.7226                & \textbf{4.5731}              & \textbf{9.8262}          \\ 

% \midrule

% \multirow{3}{*}{\textbf{MG-1}}     & MO   & \textbf{0.4929}       & 7.7544       & 3.3246       & 10.6532      & 22.2251         \\ 
%                             &\alpha = 1       & 0.6134            & 2.7401               & 2.7606                & 5.7572              & 11.8713         \\ 
%                                 & \alpha = 10       & 0.6127            & 2.1461               & \textbf{2.7283}                & 4.9880              & 10.4751         \\ 
%                                 & \alpha = 50       & 0.6129            & \textbf{2.0078}               & 2.7286                & \textbf{4.8814}              & \textbf{10.2307 }        \\ 

% \midrule

% \multirow{3}{*}{\textbf{MG-2}}      & MO   & \textbf{0.4989}       & 12.2648      & 4.7484       & 15.9152      & 33.4273         \\ 
%                             & \alpha = 1       & 0.6155            & 2.5696               & 2.8015                & 5.0190              & 11.0057         \\ 
%                                 & \alpha = 10      & 0.6139            & 2.1411               & 2.7531                & 4.8689              & 10.3769         \\ 
%                                 & \alpha = 50      & 0.6136            & \textbf{2.0096}               & \textbf{2.7364}                & \textbf{4.7566}              & \textbf{10.1161}         \\ 

% \bottomrule
% \end{tabular}
% \label{tab:rmse_error}
% \end{table*}
